Sparse Bayesian Learning with Dynamic Filtering for Inference of Time-Varying Sparse Signals

Many signal processing applications require estimation of time-varying sparse signals, potentially with the knowledge of an imperfect dynamics model. In this paper, we propose an algorithm for dynamic filtering of time-varying sparse signals based on the sparse Bayesian learning (SBL) framework. The key idea underlying the algorithm, termed SBL-DF, is the incorporation of a signal prediction generated from a dynamics model and estimates of previous time steps into the hyperpriors of the SBL probability model. The proposed algorithm is robust to imperfect dynamics models (due to the propagation of dynamics information through higher-order statistics), robust to certain undesirable dictionary properties such as coherence (due to properties of the SBL framework), allows the use of arbitrary dynamics models, and requires the tuning of fewer parameters than many other dynamic filtering algorithms do. We also extend the fast marginal likelihood SBL inference procedure to the informative hyperprior setting to create a particularly efficient version of the SBL-DF algorithm. Numerical simulations show that SBL-DF converges much faster and to more accurate solutions than standard SBL and other dynamical filtering algorithms. In particular, we show that SBL-DF outperforms state of the art algorithms when the dictionary contains challenging structure such as coherence and column scaling, as is found in many practical applications.

==> sec_derivations.tex <==
% !TeX root = dynamicsbl.tex

\subsection{Background and related work}
\label{sec:derivations-background}

\subsubsection{Marginal log-likelihood}

Using the fact that $p(\log z) = z~p(z)$,
\begin{align}
	p(\log \gamma_i) &= \gamma_i b_i^{a_i} \Gamma^{-1}(a_i) \gamma_i^{-a_i-1} e^{- b_i \gamma_i^{-1}} \\
	&= b_i^{a_i} \Gamma^{-1}(a_i) \gamma_i^{-a_i} e^{- b_i \gamma_i^{-1}} \\
	\log p(\log \gamma_i) &= a_i \log b_i + \log \Gamma^{-1}(a_i) - a_i \log \gamma_i - b_i \gamma_i^{-1} \\
	&= a_i \log \gamma_i^{-1} - b_i \gamma_i^{-1} + \mathrm{const} \\
	p(\log \noisevar) &= \noisevar d^c \Gamma^{-1}(c) \noisevar^{-c-1} e^{-d \lambda^{-1}} \\
	&= d^c \Gamma^{-1}(c) \noisevar^{-c} e^{-d \noisevar^{-1}} \\
	\log p(\log \noisevar) &= c \log d + \log \Gamma^{-1}(c) - c \log \lambda - d \lambda^{-1} \\
	&= c \log \noisevar^{-1} - d \noisevar^{-1} + \mathrm{const} \\
	\log p(\y \vert \log \g, \log \noisevar) &= -\frac{N}{2} \log 2 \pi - \frac{1}{2} \log \abs{\Sy} - \frac{1}{2} \y^T \Sy^{-1} \y \\
	\Rightarrow
	\log \mathcal{L}(\g,\noisevar) &= \log p(\y \vert \log \g, \log \noisevar) + \sum_{i=1}^N \log p(\log \gamma_i) + \log p(\log \noisevar) \\
	&\propto -\frac{1}{2} \log \abs{\Sy} - \frac{1}{2} \y^T \Sy^{-1} \y + \sum_{i=1}^N \left( a_i \log \gamma_i^{-1} - b_i \gamma^{-1} \right) + c \log \noisevar^{-1} - d \noisevar^{-1}.
\end{align}

\subsection{Dynamic filtering via sparse Bayesian learning (SBL-DF)}

\subsubsection{Map from dynamics estimate to hyperparameters}

We first derive the value $\g_{\mathrm{dyn}}$ that minimizes $\E\left[\norm{\widehat{\x}-\widetilde{\x}}_2^2\right]$. Note that from the SBL posterior mean expression (\ref{eq:sbl-point-estimate}) we have $\widehat{\x} = \left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\y$ and from the measurement model (\ref{eq:meas-model}) we have $\y = \P\x + \e$. (We assume $\x = \widetilde{\x}$ \mattcomment{(TODO---justify)}.) Define the following quantities:
\begin{align}
\bm{G} &= \P^T\P \\
\D &= \left(\lambda\G^{-1}+\bm{G}\right)^{-1} \\
\A &= \left(\lambda\G^{-1}+\P^T\P\right)^{-1} \P^T\P - \I = \D \bm{G} - \bm{I} \\
\widetilde{\e} &= \D\P^T\e
\end{align}
where $\bm{G}$ (and therefore $\D$ and $\A$) are diagonal when $\P$ has orthogonal columns. Also, note that because $\e \sim \N\left(\bm{0},\noisevar\bm{I}\right)$ and it is a fact that $\mathrm{Cov}\left[\bm{\Psi}\x\right] = \bm{\Psi}\mathrm{Cov}\left[\x\right]\bm{\Psi}^T$, and for $x \sim \N\left(\bm{\mu},\bm{\Sigma}\right)$ we have $\E\left[\x\x^T\right] = \bm{\Sigma} + \bm{\mu}\bm{\mu}^T$ (see \cite{petersen2012matrix}), we have
\begin{align}
\et &\sim \N\left(\bm{0}, \noisevar \D\bm{G}\D^T\right) \\
\E\left[\et\et^T\right] &= \E\left[\D\P^T\e\e^T\P\D\right] \\
&= \D\P^T\E\left[\e\e^T\right]\P\D^T \\
&= \noisevar\D\P^T\P\D^T \\
&= \noisevar\D\bm{G}\D^T
\end{align}

Therefore,
\begin{align}
\E\left[\norm{\widehat{\x}-\x}_2^2\right] &= \E\left[\norm{\left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\y - \x}_2^2\right] \\
&= \E\left[\norm{\left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\P\x + \left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\e - \x}_2^2\right] \\
&= \E\left[\norm{\D\bm{G}\x + \D\P^T\e - \x}_2^2\right] \\
&= \E\left[\norm{\left(\D\bm{G}-\I\right)\x + \D\P^T\e}_2^2\right] \\
&= \E\left[\norm{\A\x + \et}_2^2\right] \\
&= \E\left[\x^T\A^T\A\x + 2 \x^T\A^T\et + \et^T\et\right] \\
&= \x^T\A^T\A\x + 2\x^T\A^T\E\left[\et\right] + \E\left[\et^T\et\right] \\
&= \x^T\A^T\A\x + \E\left[\et^T\et\right] \\
&= \x^T\A^T\A\x + \mathrm{Tr}\left[\E\left[\et\et^T\right]\right] \\
&= \x^T\A^T\A\x + \noisevar\mathrm{Tr}\left[\D\bm{G}\D^T\right]
\end{align}

Assuming $\G$ is symmetric (as is the case in SBL), calculating the derivative and setting to zero gives
\begin{align}
%\frac{\partial}{\partial\g} \left[ \lambda \G^{-1} + \bm{B} \right] &= -\G^{-2} \\
%\frac{\partial}{\partial\g} \left[ \left( \lambda \G^{-1} + \bm{B} \right)^{-1} \right] &= \frac{\partial}{\partial\left(\lambda\G^{-1}+\bm{B}\right)} \left[ \left(\lambda\G^{-1}+\B\right)^{-1} \right] \times \frac{\partial}{\partial\g} \left[ \lambda \G^{-1} + \B \right] \\
%&= \left[ -\left(\lambda\G^{-1}+\B\right)^{-1} \frac{\partial\left(\lambda\G^{-1}+\B\right)}{\partial\g} \left(\lambda\G^{-1}+\B\right)^{-1} \right] \times \left[ - \G^{-2} \right] \\
%&= \left[ -\left(\lambda\G^{-1}+\B\right)^{-1} \left(-\G^{-2}\right) \left(\lambda\G^{-1}+\B\right)^{-1} \right] \times \left[ - \G^{-2} \right] \\
%&= \left(\lambda\G^{-1}+\B\right)^{-1} \G^{-2} \left(\lambda\G^{-1}+\B\right)^{-1} \G^{-2} \\
%&= \D \G^{-2} \D \G^{-2} \\
%\frac{\partial}{\partial\g} \left[ \sigma^2\D\B\D^T \right] &= \frac{\partial}{\partial \D} \left[ \sigma^2\D\B\D^T \right] \times \frac{\partial}{\partial\left(\lambda\G^{-1}+\bm{B}\right)} \left[ \left(\lambda\G^{-1}+\B\right)^{-1} \right] \times \frac{\partial}{\partial\g} \left[ \lambda \G^{-1} + \B \right] \\
%&= \left( \D + \D^T \right) \times \D \G^{-2} \D \G^{-2} \\
%&= \D^2 \G^{-2} \D \G^{-2} + \D^T \D \G^{-2} \D \G^{-2} \\
%&= TODO
0 &= \frac{\partial}{\partial\G^{-1}} \E\left[\norm{\widehat{\x}-\x}_2^2\right] \\
&= \frac{\partial}{\partial\G^{-1}} \left[ \x^T\A^T\A\x + \noisevar\mathrm{Tr}\left[\D\bm{G}\D^T\right] \right] \\
&= -2\lambda\D^T\bm{G}\x\x^T\A^T\D^T - 2\lambda\noisevar\D\D^T\bm{G}\D \\
&= \D^T\bm{G}\x\x^T\A^T\D^T + \noisevar\D\D^T\bm{G}\D \\
&= \D\bm{G}\x\x^T\A\D + \noisevar\D\D\bm{G}\D \\
&= \D \bm{G} \left( \x\x^T\A + \noisevar\D \right) \D \\
&= \D \bm{G} \left[ \x\x^T \left( \D \bm{G} - \I \right) + \noisevar \D \right] \D
\end{align}

We now need to make further assumptions to simplify further, and do so by assuming that $\bm{G} = \P^T\P$ is diagonal (i.e., $\P$ has orthogonal columns, but might not necessarily be orthonormal). Then, denoting $g_i = \bm{G}_{ii}$, we have
\begin{align}
\E \left[ \norm{\widehat{\x}-\x}_2^2 \right] &= \sum_{i=1}^N \left[ \left(\frac{g_i}{\noisevar\gamma_i^{-1}+g_i} - 1\right)^2 x_i^2 + \noisevar \frac{g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^2} \right] \\
&= \sum_{i=1}^N \left[ \frac{\noisevar^2 \gamma_i^{-2}}{\left(\noisevar\gamma_i^{-1}+g_i\right)^2} x_i^2 + \noisevar \frac{g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^2} \right] \\
&= \sum_{i=1}^N \frac{\noisevar^2 \gamma_i^{-2} x_i^2 + \noisevar g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^2} \\
\end{align}
and then
\begin{align}
\frac{\partial}{\partial\g^{-1}} \E \left[ \norm{\widehat{\x}-\x}_2^2 \right] &= \sum_{i=1}^N \frac{\partial}{\partial\gamma_i^{-1}} \left[ \frac{\noisevar^2\gamma_i^{-2}x_i^2 + \noisevar g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^2} \right] \\
&= \frac{\frac{\partial}{\partial\gamma_i^{-1}}\left[\noisevar^2\gamma_i^{-2}x_i^2+\sigma^2g_i\right] \left(\noisevar\gamma_i^{-1}+g_i\right)^2 - \left(\noisevar^2\gamma_i^{-2}x_i^2+\noisevar g_i\right)\frac{\partial}{\partial\gamma_i^{-1}}\left[\left(\noisevar\gamma_i^{-1}+g_i\right)^2\right]}{\left(\noisevar\gamma_i^{-1}+g_i\right)^4} \\
&= \frac{\left(2\noisevar^2\gamma_i^{-1}x_i^2\right) \left(\noisevar\gamma_i^{-1}+g_i\right)^2 - \left(\noisevar^2\gamma_i^{-2}x_i^2+\sigma^2g_i\right)\left(2\noisevar^2\gamma_i^{-1}+2\noisevar g_i\right)}{\left(\noisevar\gamma_i^{-1}+g_i\right)^4} \\
&= 2\noisevar \frac{\left(\noisevar\gamma_i^{-1}x_i^2\right) \left(\noisevar\gamma_i^{-1}+g_i\right)^2 - \left(\noisevar^2\gamma_i^{-2}x_i^2+\sigma^2g_i\right)\left(\noisevar\gamma_i^{-1}+g_i\right)}{\left(\noisevar\gamma_i^{-1}+g_i\right)^4} \\
&= 2\noisevar \frac{\left(\noisevar\gamma_i^{-1}x_i^2\right) \left(\noisevar\gamma_i^{-1}+g_i\right) - \left(\noisevar^2\gamma_i^{-2}x_i^2+\sigma^2g_i\right)}{\left(\noisevar\gamma_i^{-1}+g_i\right)^3} \\
&= 2\noisevar \frac{\noisevar\gamma_i^{-1}g_ix_i^2 - \noisevar g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^3}.
\end{align}
Setting to zero and solving yields
\begin{align}
0 &= 2\noisevar^2 \frac{\gamma_i^{-1}g_ix_i^2 - g_i}{\left(\noisevar\gamma_i^{-1}+g_i\right)^3} \\
&= \gamma_i^{-1}g_ix_i^2 - g_i \\
\gamma_i^{-1}g_ix_i^2 &= g_i \\
\gamma_i^* &= x_i^2.
\end{align}

The value $\g^*$ that minimizes the dynamics portion of the SBL objective $\ell_{\mathrm{dyn}}\left(\g,\lambda\right)$ (\ref{eq:sbl-objective-dyn}) is
\begin{align}
0 &= \frac{\partial}{\partial \gamma_i} \left( b_i \gamma_i^{-1} + a_i \log \gamma_i \right) \\
&= -b_i \gamma_i^{-2} + a_i \gamma_i^{-1} \\
&= -b_i + a_i \gamma_i \\
\Rightarrow \gamma_i^* &= \frac{b_i}{a_i}.
\end{align}

\subsubsection{Effective SBL prior}

\begin{align}
	p(x_i \vert a_i, b_i) &= \int_0^{\infty} p(x_i \vert \gamma_i) p(\gamma_i \vert a_i, b_i) d\gamma_i \\
	&= \int_0^\infty \frac{1}{\sqrt{2\pi\gamma_i}} \exp\left(-\frac{x_i^2}{2\gamma_i}\right)\frac{b_i^{a_i}}{\Gamma(a_i)} \gamma_i^{-a_i-1} e^{-b_i \gamma_i^{-1}} d\gamma_i \\
	&= \frac{b_i^{a_i}}{\sqrt{2\pi}\Gamma(a_i)} \int_0^\infty \gamma_i^{-a_i-\tfrac{3}{2}} \exp \left[ - \left(\frac{x_i^2}{2}+b_i\right) \gamma_i^{-1} \right] d\gamma_i \\
	\intertext{Letting $\kappa_i = \gamma_i^{-1}$ (so $d\gamma_i = -\kappa_i^{-2} d\kappa_i$),}
	&= \frac{b_i^{a_i}}{\sqrt{2\pi}\Gamma(a_i)} \int_\infty^0 \kappa_i^{a_i+\tfrac{3}{2}} \exp\left[-\left(b_i+\frac{x_i^2}{2}\right)\kappa_i\right] \left(-\kappa_i^{-2} d\kappa_i\right) \\
	&= \frac{b_i^{a_i}}{\sqrt{2\pi}\Gamma(a_i)} \int_0^\infty \kappa_i^{a_i-\tfrac{1}{2}} \exp\left[-\left(b_i+\frac{x_i^2}{2}\right)\kappa_i\right] d\kappa_i \\
	\intertext{Using the well-known definite integral $\int_0^\infty x^n e^{-cx} dx = \frac{\Gamma(n+1)}{c^{n+1}}$ with $n = a_i-\frac{1}{2}$ and $c = b_i+\frac{x_i^2}{2}$,}
	&= \frac{b_i^{a_i} \Gamma(a_i + \tfrac{1}{2})}{\sqrt{2\pi} \Gamma(a_i)} \left( b_i + \frac{x_i^2}{2} \right)^{-\left(a_i + \tfrac{1}{2}\right)}
\end{align}

\subsubsection{Parameterization of effective SBL prior as non-standardized Student's-t}

\begin{align}
	\frac{\Gamma\left(\frac{\nu+1}{2}\right)}{\Gamma\left(\frac{\nu}{2}\right) \sqrt{\pi\nu} \sigma} \left( 1 + \frac{1}{\nu} \frac{x^2}{\sigma} \right)^{-\frac{\nu+1}{2}} &= \frac{\Gamma\left(\frac{2a+1}{2}\right)}{\Gamma\left(a\right) \sqrt{2\pi a} \sqrt{b/a}} \left( 1 + \frac{1}{2a}\frac{x^2}{b a^{-1}} \right)^{-\left(a+\tfrac{1}{2}\right)} \\
	&= \frac{\Gamma\left(a+\frac{1}{2}\right)}{\sqrt{2\pi} \Gamma(a) \sqrt{b}} \frac{b^{-\left(a+\tfrac{1}{2}\right)}}{b^{-a} b^{-1/2}} \left( 1 + \frac{x^2}{2b} \right)^{-\left(a+\tfrac{1}{2}\right)} \\
	&= \frac{b^a \Gamma\left(a+\frac{1}{2}\right)}{\sqrt{2\pi}\Gamma\left(a\right)} \left( b + \frac{x^2}{2} \right)^{-\left(a+\tfrac{1}{2}\right)}
\end{align}

\subsubsection{Decomposition of SBL objective}

Using the fact that $\abs{\bm{A} + \bm{B} \bm{C}} = \abs{\bm{A}} \abs{\bm{I} + \bm{C} \bm{A}^{-1} \bm{B}}$ for invertible $\bm{A}$, we can decompose the determinant $\bm{C}$ in the log-likelihood $\mathcal{L}(\g,\noisevar)$ as
\begin{align}
\left| \bm{C} \right| &= \left| \bm{C}_{-j} + \gamma_j \bm{\phi}_j \bm{\phi}_j^T \right| \\
&= \left| \bm{C}_{-j} \right| \left| 1 + \gamma_j \bm{\phi}_j^T \bm{C}^{-1}_{-j} \bm{\phi}_j \right|.
\end{align}

Similarly, using the Woodbury identity we can decompose the inverse $\bm{C}^{-1}$ in the log-likelihood $\mathcal{L}(\g,\noisevar)$ as
\begin{align}
\bm{C}^{-1} &= \left( \bm{C}_{-j} + \gamma_j \bm{\phi}_j \bm{\phi}_j^T \right)^{-1} \\
&= \bm{C}_{-j}^{-1} - \bm{C}_{-j}^{-1} \bm{\phi}_j \left( \gamma_j^{-1} + \bm{\phi}_j^T \bm{C}_{-j}^{-1} \bm{\phi}_j \right)^{-1} \bm{\phi}_j^T \bm{C}_{-j}^{-1} \\
&= \bm{C}_{-j}^{-1} - \frac{\bm{C}_{-j}^{-1} \bm{\phi}_j \bm{\phi}_j^T \bm{C}_{-j}^{-1}}{\gamma_j^{-1} + \bm{\phi}_j^T \bm{C}_{-j}^{-1} \bm{\phi}_j}. \label{eq:Cinv-decomp}
\end{align}

Substituting these expressions into the hyperparameter posterior log-likelihood (\ref{eq:sbl-marginal-log-likelihood}) and separating the terms involving $\gamma_j$ from those involving $\g_{-j}$ and $\noisevar$, we can decompose the negative log-likelihood (\ref{eq:sbl-objective}) as (\ref{eq:sbl-fml-objective-decomp}), which is a sum of the terms excluding element $j$ (\ref{eq:sbl-fml-lgammanoj}) and the terms involving element $j$ (\ref{eq:sbl-fml-lgammaj}),
\begin{align}
	\ell(\gamma_j) &= \log \left| 1 + \gamma_j \bm{\phi}_j \bm{C}_{-j}^{-1} \bm{\phi}_j^T \right| - \y^T \frac{\bm{C}_{-j}^{-1} \bm{\phi}_j \bm{\phi}_j^T \bm{C}_{-j}^{-1}}{\gamma_j^{-1} + \bm{\phi}_j \bm{C}_{-j}^{-1} \bm{\phi}_j} \y - 2 \left( a_j \log \gamma_j^{-1} - b_j \gamma_j^{-1} \right) \\
	&= \log \left| \gamma_j \right| + \log \left| \gamma_j^{-1} + \bm{\phi}_j \bm{C}_{-j}^{-1} \bm{\phi}_j^T \right| - \y^T \frac{\bm{C}_{-j}^{-1} \bm{\phi}_j \bm{\phi}_j^T \bm{C}_{-j}^{-1}}{\gamma_j^{-1} + \bm{\phi}_j \bm{C}_{-j}^{-1} \bm{\phi}_j} \y - 2 \left( a_j \log \gamma_j^{-1} - b_j \gamma_j^{-1} \right) \notag \\
	&= - \log \gamma_j^{-1} + \log \left( \gamma_j^{-1} + s_j \right) - \frac{q_j^2}{\gamma_j^{-1} + s_j} - 2 a_j \log \gamma_j^{-1} + 2 b_j \gamma_j^{-1}
\end{align}
where, following the notation of \cite{tipping2003fast}, $s_j = \bm{\phi}_j^T \bm{C}_{-j}^{-1} \bm{\phi}_j$ and $q_j = \bm{\phi}_j^T \bm{C}_{-j}^{-1} \y$.

\subsubsection{First derivative of likelihood}

\begin{align}
	\frac{\partial \ell(\gamma_j)}{\partial \gamma_j} &= \gamma_j^{-1} - \frac{1}{\gamma_j^2 s_j + \gamma_j} - \frac{q_j^2}{(1+\gamma_j s_j)^2} + 2 a_j \gamma_j^{-1} - 2 b_j \gamma_j^{-2} \\
	&= \frac{1}{\left(1+\gamma_js_j\right)^2} \left[ \gamma_j^{-1} \left(1+\gamma_js_j\right)^2 - \gamma_j^{-1}\left(1+\gamma_js_j\right) - q_j^2 + 2a_j\gamma_j^{-1}\left(1+\gamma_js_j\right)^2 - 2b_j\gamma_j^{-2}\left(1+\gamma_js_j\right)^2\right] \\
	&= \frac{1}{\left(1+\gamma_js_j\right)^2} \left[ \gamma_j^{-1} + 2s_j + \gamma_js_j^2 - \gamma_j^{-1} - s_j - q_j^2 + 2a_j\gamma_j^{-1}\left(1+2\gamma_js_j+\gamma_j^2s_j^2\right) - 2b_j\gamma_j^{-2}\left(1+2\gamma_js_j+\gamma_j^2s_j^2\right) \right] \\
	&= \frac{1}{\left(1+\gamma_js_j\right)^2} \left[ s_j + \gamma_j s_j^2 - q_j^2 + 2a_j\gamma_j^{-1} + 4a_js_j + 2a_j\gamma_js_j^2 - 2b_j\gamma_j^{-2} - 4\gamma_j^{-1}b_js_j - 2b_js_j^2 \right] \\
	&= \frac{1}{\gamma_j^2 \left(1+\gamma_js_j\right)^2} \left[ s\gamma_j^2 + s_j^2 \gamma_j^3 - q_j^2 \gamma_j^2 + 2a_j\gamma_j + 4a_js_j\gamma_j^2 + 2a_js_j^2\gamma_j^3 - 2b_j - 4b_js_j\gamma_j - 2b_js_j^2\gamma_j^2 \right] \\
	&= \frac{2 s_j^{-2}}{\gamma_j^2 \left(\gamma_j+s_j^{-1}\right)^2} \left[ \left(\frac{1}{2}s_j^2+a_js_j^2\right)\gamma_j^3 + \left(\frac{1}{2}s_j-\frac{1}{2}q_j^2+2a_js_j-b_js_j^2\right)\gamma_j^2 + \left(a_j-2b_js_j\right)\gamma_j - b_j \right].
\end{align}

\subsubsection{Second derivative of likelihood}

\begin{align}
	\frac{\partial^2 \ell(\gamma_j)}{\partial \gamma_j^2} &= -\gamma_j^{-2} + \frac{2\gamma_js_j+1}{\left(\gamma_j^2s_j+\gamma_j\right)^2} + \frac{2q_j^2s_j}{\left(\gamma_js_j+1\right)^3} - 2a_j\gamma_j^{-2} + 4b_j\gamma_j^{-3} \\
	&= - \frac{\left(\gamma_js_j+1\right)^2}{\gamma_j^2\left(\gamma_js_j+1\right)^2} + \frac{2\gamma_js_j+1}{\gamma_j^2\left(\gamma_js_j+1\right)^2} + \frac{2q_j^2s_j}{\left(\gamma_js_j+1\right)^3} - 2a_j\gamma_j^{-2} + 4b_j\gamma_j^{-3} \\
	&= \frac{-\gamma_j^2s_j^2-2\gamma_js_j-1+2\gamma_js_j+1}{\gamma_j^2\left(\gamma_js_j+1\right)^2} + \frac{2q_j^2s_j}{\left(\gamma_js_j+1\right)^3} - 2a_j\gamma_j^{-2} + 4b_j\gamma_j^{-3} \\
	&= -\frac{s_j^2}{\left(\gamma_js_j+1\right)^2} + \frac{2q_j^2s_j}{\left(\gamma_js_j+1\right)^3} - 2a_j\gamma_j^{-2} + 4b_j\gamma_j^{-3} \\
	&= \frac{-s_j^2\left(\gamma_js_j+1\right)+2q_j^2s_j}{\left(\gamma_js_j+1\right)^3} - 2a_j\gamma_j^{-2} + 4b_j\gamma_j^{-3} \\
	&= -2 a_j \gamma_j^{-2} + 4b_j\gamma_j^{-3} - \frac{s_j^3\gamma_j+s_j^2-2q_j^2s_j}{\left(\gamma_js_j+1\right)^3},
\end{align}

\subsubsection{Simplified expressions for $s_i$ and $q_i$}

\begin{align}
s_i &= \bm{\phi}_i^T \bm{C}_{-i}^{-1} \bm{\phi}_i \\
&= \bm{\phi}_i \left( \bm{C}^{-1} + \frac{\bm{C}_{-i}^{-1} \bm{\phi}_i \bm{\phi}_i^T \bm{C}_i^{-1}}{\gamma_i^{-1} + \bm{\phi}_i^T \bm{C}_{-i}^{-1} \bm{\phi}_i} \right) \bm{\phi}_i \\
&= S_i + \frac{s_i^2}{\gamma_i^{-1} + s_i} \\
s_i \gamma_i^{-1} + s_i^2 &= s_i^2 + S_i \gamma_i^{-1} + S_i s_i \\
s_i \left( \gamma_i^{-1} - S_i \right) &= S_i \gamma_i^{-1} \\
s_i &= \frac{S_i \gamma_i^{-1}}{\gamma_i^{-1} - S_i} \\
&= \frac{S_i}{1 - \gamma_i S_i} \\
q_i &= \bm{\phi}_i^T \bm{C}_{-1}^{-1} \y \\
&= \bm{\phi}_i^T \left( \bm{C}^{-1} + \frac{\bm{C}_{-i}^{-1} \bm{\phi}_i \bm{\phi}_i^T \bm{C}_{-i}^{-1}}{\gamma_i^{-1} + \bm{\phi}_i^T \bm{C}_{-i}^{-1}\bm{\phi}_i} \right) \y \\
&= Q_i + \frac{s_i q_i}{\gamma_i^{-1} + s_i} \\
q_i \left( \gamma_i^{-1} + s_i \right) &= Q_i \left( \gamma_i^{-1} + s_i \right) + s_i q_i \\
q_i \gamma_i^{-1} &= Q_i \gamma_i^{-1} + Q_i s_i \\
q_i &= Q_i + Q_i s_i \gamma_i \\
&= Q_i \left( 1 + s_i \gamma_i \right) \\
&= Q_i + \frac{Q_i \gamma_i S_i}{1 - \gamma_i S_i} \\
&= Q_i \left( 1 + \frac{\gamma_i S_i}{1 - \gamma_i S_i} \right) \\
&= Q_i \left( \frac{1}{1 - \gamma_i S_i} \right) \\
&= \frac{Q_i}{1-\gamma_iS_i}
\end{align}

\subsubsection{Bound for $y^TC^{-1}y$}

First, note that the solution to
\begin{equation}
	\underset{\x}{\arg\min}~\frac{1}{\lambda} \norm{\y-\P\x}_2^2 + \norm{\G^{-1/2}\x}_2^2
\end{equation}
is
\begin{align}
	0 &= \nabla_{\x} \left[ \frac{1}{\lambda} \norm{\y-\P\x}_2^2 + \norm{\G^{-1/2}\x}_2^2 \right] \\
	&= - 2\P^T\y + 2\P^T\P \x_* + 2 \lambda \G^{-1} \x_* \\
	\Rightarrow \x_* &= \left(\P^T\P + \lambda\G^{-1}\right)^{-1} \P^T \y
\end{align}
and so returning to $\y^T\Sy^{-1}\y$ we have
\begin{align}
	\y^T\Sy^{-1}\y &= \y^T \left(\lambda\bm{I} - \P\G\P^T\right)^{-1} \y \\
	&= \lambda^{-1} \y^T \left[ \bm{I} - \P \left( \lambda \G^{-1} + \P^T\P \right)^{-1} \P^T \right] \y \\
	&= \lambda^{-1}\y^T\y - 2\lambda^{-1}\y^T\P\left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\y + \lambda^{-1}\y^T\P\left(\lambda\G^{-1}+\P^T\P\right)^{-1}\P^T\y \\
	&= \lambda^{-1}\y^T\y - 2\lambda^{-1}\y^T\P\x_* + \lambda^{-1}\x_*^T\left(\P^T\P+\lambda\G^{-1}\right)\x_* \\
	&= \lambda^{-1}\left[\y^T\y - 2\y^T\P\x_* + \x_*^T\P^T\P\x_*\right] + \x_*^T\G^{-1}\x_* \\
	&= \frac{1}{\lambda} \norm{\y-\P\x_*}_2^2 + \norm{\G^{-1/2}\x_*}_2^2 \\
	&= \underset{\x}{\arg\min}~\frac{1}{\lambda} \norm{\y-\P\x}_2^2 + \norm{\G^{-1/2}\x}_2^2
\end{align}
and therefore
\begin{equation}
	\y^T\Sy^{-1}\y + 2\sum_ib_i\gamma_i^{-1} = \underset{\x}{\arg\min}~\frac{1}{\lambda} \norm{\y-\P\x}_2^2 + \norm{\G^{-1/2}\x}_2^2 + 2\sum_ib_i\gamma_i^{-1}
\end{equation}

\subsubsection{Optimal value of majorizing function}

\begin{align}
	\frac{\partial \log \abs{\Sy}}{\partial \gamma_i} &= \frac{\partial}{\partial \gamma_i} \log \det \left( \lambda \bm{I} + \bm{\Phi} \G \bm{\Phi}^T \right) \\
	\intertext{From \cite{petersen2012matrix},}
	&= \mathrm{Tr} \left[ \Sy^{-1} \frac{\partial}{\partial \gamma_i} \left( \lambda \bm{I} + \bm{\Phi} \bm{\Gamma} \bm{\Phi}^T \right) \right] \\
	&= \mathrm{Tr} \left[ \Sy^{-1} \frac{\partial}{\partial \gamma_i} \left( \bm{\Phi} \bm{\Gamma} \bm{\Phi}^T \right) \right] \label{eq:dlogdetSy-incomplete}
\end{align}

We evaluate $\frac{\partial}{\partial \gamma_i} \bm{\Phi} \G \bm{\Phi}^T$ element-wise:
\begin{align}
	\P \G \P^T &= \begin{bmatrix} \sum_k \Phi_{1k} \gamma_k \Phi_{1k} & \sum_k \Phi_{1k} \gamma_k \Phi_{2k} & \dots & \sum_k \Phi_{1k} \gamma_k \Phi_{nk} \\ \sum_k \Phi_{2k} \gamma_k \Phi_{1k} & \ddots & & \vdots \\ \vdots & & & \\ \sum_k \Phi_{nk} \gamma_k \Phi_{1k} & \dots & & \sum_k \Phi_{nk} \gamma_k \Phi_{nk} \end{bmatrix} \\
	\Rightarrow \quad \frac{\partial \P \G \P^T}{\partial \gamma_i} &= \begin{bmatrix} \Phi_{1i} \Phi_{1i} & \Phi_{1i} \Phi_{2i} & \dots & \Phi_{1i} \Phi_{ni} \\ \Phi_{2i} \Phi_{1i} & \ddots & & \vdots \\ \vdots & & & \\ \Phi_{ni} \Phi_{1i} & \dots & & \Phi_{ni} \Phi_{ni} \end{bmatrix} \\
	&= \bm{\phi}_i \bm{\phi}_i^T
\end{align}

Substituting this into the expression for the gradient of $\log \lvert \Sy \rvert$ in (\ref{eq:dlogdetSy-incomplete}) gives us
\begin{align}
	\frac{\partial \log \abs{\Sy}}{\partial \gamma_i} &= \mathrm{Tr} \left[ \Sy^{-1} \bm{\phi}_i \bm{\phi_i}^T \right] \\
	&= \mathrm{Tr} \left[ \bm{\phi}_i^T \Sy^{-1} \bm{\phi}_i \right] \\
	&= \bm{\phi}_i^T \Sy^{-1} \bm{\phi} \\
	&= \left[ \P^T \Sy^{-1} \P \right]_{ii}
\end{align}
so
\begin{equation}
	\z_{\mathrm{opt}} = \nabla_{\g} \log \abs{\Sy} = \mathrm{diag}\left[ \P^T \Sy^{-1} \P. \right]
\end{equation}

\subsection{Details of fast marginal likelihood}

\subsubsection{Efficient initializations of $\left\{S_i\right\}$ and $\left\{Q_i\right\}$}

\begin{align}
	S_k &= \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \bm{\phi}_i \widetilde{\gamma_i} \bm{\phi}_i^T \right)^{-1} \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \bm{\phi}_i \left( \gamma_i^{-1} + \sigma^{-2} \bm{\phi}_i^T \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \right] \bm{\phi}_k \notag \\
	&= \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_k - \sigma^{-4} \bm{\phi}_k^T \bm{\phi}_i \Sxy \bm{\phi}_i^T \bm{\phi}_k \\
	Q_k &= \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \bm{\phi}_i \widetilde{\gamma_i} \bm{\phi}_i^T \right)^{-1} \y \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \bm{\phi}_i \left( \gamma_i^{-1} + \sigma^{-2} \bm{\phi}_i^T \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \right] \y \notag \\
	&= \sigma^{-2} \bm{\phi}_k^T \y - \sigma^{-4} \bm{\phi}_k^T \bm{\phi}_i \Sxy \bm{\phi}_i^T \y
\end{align}

\subsubsection{Efficient updates for re-estimating an element}

\begin{align}
	\Sxy^{(\mathrm{new})} &= \left( \G^{-1} - \e_i\gamma_i^{-1}\e_i^T + \e_i\widetilde{\gamma_i}^{-1}\e_i^T + \lambda^{-1} \P^T\P \right)^{-1} \\
	&= \left( \G^{-1} + \lambda^{-1} \P^T\P + \e_i\left(\widetilde{\gamma_i}^{-1}-\gamma_i^{-1}\right)\e_i^T \right)^{-1} \\
	&= \left( \Sxy^{-1} + \e_i\left(\widetilde{\gamma_i}^{-1}-\gamma_i^{-1}\right)\e_i^T \right)^{-1} \\
	&= \Sxy - \left(\Sxy\right)_i \left( \frac{1}{\widetilde{\gamma_i}^{-1}-\gamma_i^{-1}} + \left(\Sxy\right)_{ii}\right)^{-1} \left(\Sxy\right)_i^T \\
	&= \Sxy - \kappa_i \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	\muxy^{(\mathrm{new})} &= \lambda^{-1} \left[ \Sxy - \kappa_i \left(\Sxy\right)_i \left(\Sxy\right)_i^T \right] \P^T \y \\
	&= \lambda^{-1} \Sxy \P^T \y - \lambda^{-1} \kappa_i \left(\Sxy\right)_i \left(\Sxy\right)_i^T \P^T \y \\
	&= \muxy - \kappa_i \left[ \lambda^{-1} \left(\Sxy\right)_i^T \P^T \y \right] \left( \Sxy \right)_i \\
	&= \muxy - \kappa_i \left( \muxy \right)_i \left( \Sxy \right)_i \\
	S_k^{(\mathrm{new})} &= \bm{\phi}_k^T \left(\bm{C}^{(\mathrm{new})}\right)^{-1} \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left[ \sigma^2\bm{I} + \P\G^{(\mathrm{new})}\P^T \right]^{-1} \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{(\mathrm{new})} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy^{(\mathrm{new})} \P^T \right] \bm{\phi}_k \\
	&= \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_k - \sigma^{-4} \bm{\phi}_k^T \P \Sxy^{(\mathrm{new})} \P^T \bm{\phi}_k \\
	&= \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_k - \sigma^{-4} \bm{\phi}_k^T \P \left[ \Sxy - \kappa_i \left(\Sxy\right)_i \left(\Sxy\right)_i \right] \P^T \bm{\phi}_k \\
	&= \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_k - \sigma^{-4} \bm{\phi}_k^T \P \Sxy \P^T \bm{\phi}_k + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left( \Sxy \right)_i \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left( \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy \P^T \right) \bm{\phi}_k + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left( \Sxy \right)_i \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left( \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy \P^T \right) \bm{\phi}_k + \kappa_i \left( \sigma^{-2} \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \bm{\phi}_k + \kappa_i \left( \sigma^{-2} \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	&= \bm{\phi}_k^T \left[ \sigma^2 \bm{I} + \P \G \P^T \right]^{-1} \bm{\phi}_k + \kappa_i \left( \sigma^{-2} \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	&= \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_k + \kappa_i \left( \sigma^{-2} \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	&= S_k + \kappa_i \left( \sigma^{-2} \left( \Sxy \right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	Q_k^{(\mathrm{new})} &= \bm{\phi}_k^T \left(\bm{C}^{(\mathrm{new})}\right)^{-1} \y \\
	&= \bm{\phi}_k^T \left[ \sigma^2\bm{I} + \P\G^{(\mathrm{new})}\P^T \right]^{-1} \y \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{(\mathrm{new})} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \y \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy^{(\mathrm{new})} \P^T \right] \y \\
	&= \sigma^{-2} \bm{\phi}_k^T \y - \sigma^{-4} \bm{\phi}_k^T \P \Sxy^{(\mathrm{new})} \P^T \y \\
	&= \sigma^{-2} \bm{\phi}_k^T \y - \sigma^{-4} \bm{\phi}_k^T \P \left[ \Sxy - \kappa_i \left(\Sxy\right)_i \left(\Sxy\right)_i \right] \P^T \y \\
	&= \sigma^{-2} \bm{\phi}_k^T \y - \sigma^{-4} \bm{\phi}_k^T \P \Sxy \P^T \y + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left( \Sxy \right)_i \left( \Sxy \right)_i^T \P^T \y \\
	&= \bm{\phi}_k^T \left( \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy \P^T \right) \y + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left( \Sxy \right)_i \left( \Sxy \right)_i^T \P^T \y \\
	&= \bm{\phi}_k^T \left[ \sigma^{-2}\bm{I} - \sigma^{-4} \P \left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \y + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left(\Sxy\right)_i \left(\Sxy\right)_i^T \P^T \y \\
	&= \bm{\phi}_k^T \left[ \sigma^2 \bm{I} + \P \G \P^T \right]^{-1} \y + \sigma^{-4} \kappa_i \bm{\phi}_k^T \P \left(\Sxy\right)_i \left(\Sxy\right)_i^T \P^T \y \\
	&= \bm{\phi}_k^T \bm{C}^{-1} \y + \sigma^{-4} \kappa_i \bm{\phi}_k \P \left(\Sxy\right)_i\left(\Sxy\right)_i^T \P^T \y \\
	&= Q_k + \sigma^{-4} \kappa_i \y^T \P \left(\Sxy\right)_i \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \\
	&= Q_k + \sigma^{-4} \kappa_i \left(\Sxy\right)_i^T \P^T \y \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \\
	&= Q_k + \kappa_i \left(\muxy\right)_i \left( \sigma^{-2} \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \right)
\end{align}

\subsubsection{Efficient updates for adding an element}

\begin{align}
	\Sxy^{(\mathrm{new})} &= \left( \left[ \begin{array}{cc} \G^{-1} & \bm{0} \\ \bm{0} & \widetilde{\gamma_i} \end{array} \right] + \sigma^{-2} \left[ \begin{array}{cc} \P^T\P & \P^T\bm{\phi}_i \\ \bm{\phi}_i^T\P & \bm{\phi}_i^T\bm{\phi}_i \end{array} \right] \right)^{-1} \\
	&= \left[ \begin{array}{cc} \G^{-1} & \sigma^{-2} \P^T \bm{\phi}_i \\ \sigma^{-2} \bm{\phi}_i^T \P & \widetilde{\gamma_i} + \sigma^{-2} \bm{\phi}_i^T \bm{\phi}_i \end{array} \right]^{-1} \\
	&\triangleq \left[ \begin{array}{cc} \bm{B}_{11} & \bm{B}_{12} \\ \bm{B}_{21} & \bm{B}_{22} \end{array} \right]^{-1} \\
	\intertext{We now apply the block matrix inversion identity (see \cite[Sec.~7.4.3]{petersen2012matrix}). Defining $\bm{F}_1 = \bm{B}_{11} - \bm{B}_{12} \bm{B}_{22}^{-1} \bm{B}_{21} \in \R^{N' \times N'}$ and $\bm{F}_2 = \bm{B}_{22} - \bm{B}_{21} \bm{B}_{11}^{-1} \bm{B}_{12} \in \R$, we have}
	&= \left[ \begin{array}{cc} \bm{B}_{11} & \bm{B}_{12} \\ \bm{B}_{21} & \bm{B}_{22} \end{array} \right]^{-1} = \left[ \begin{array}{cc} \bm{F}_1^{-1} & - \bm{B}_{11}^{-1} \bm{B}_{12} \bm{F}_2^{-1} \\ -\bm{F}_{2}^{-1} \bm{B}_{21} \bm{B}_{11}^{-1} & \bm{F}_2^{-1} \end{array} \right] \\
	\intertext{These quantities can be computed as}
	\bm{F}_1^{-1} &= \left(\bm{B}_{11} - \bm{B}_{12} \bm{B}_{22}^{-1} \bm{B}_{21} \right)^{-1} \\
	&= \bm{B}_{11}^{-1} + \bm{B}_{11}^{-1} \bm{B}_{12} \bm{F}_2^{-1} \bm{B}_{21} \bm{B}_{11}^{-1} \\
	&= \Sxy + \Sxy \left( \sigma^{-2} \P^T \bm{\phi}_i \right) \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \left( \sigma^{-2} \bm{\phi}_i^T \P \right) \Sxy \\
	&= \Sxy + \sigma^{-4} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy \\
	\bm{F}_2^{-1} &= \left[ \widetilde{\gamma_i}^{-1} + \sigma^{-2} \bm{\phi}_i^T \bm{\phi}_i - \sigma^{-4} \bm{\phi}_i \P \left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \bm{\phi}_i \right]^{-1} \\
	&= \left[ \widetilde{\gamma_i}^{-1} + \bm{\phi}_i^T \left( \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{-1} + \sigma^{-2} \P^T\P \right)^{-1} \P^T \right) \bm{\phi}_i \right]^{-1} \\
	&= \left[ \widetilde{\gamma_i}^{-1} + \bm{\phi}_i^T \left( \sigma^2 \bm{I} + \P \G \P^T \right)^{-1} \bm{\phi}_i \right]^{-1} \\
	&= \left[ \widetilde{\gamma_i}^{-1} + \bm{\phi}_i^T \bm{C}^{-1} \bm{\phi}_i \right]^{-1} \\
	&= \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \\
	-\bm{B}_{11}^{-1} \bm{B}_{12} \bm{F}_2^{-1} &= -\left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \left( \sigma^{-2} \P^T \bm{\phi}_i \right) \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \\
	&= - \Sxy \sigma^{-2} \P^T \bm{\phi}_i \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \\
	&= - \sigma^{-2} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \Sxy \P^T \bm{\phi}_i \\
	-\bm{F}_2^{-1} \bm{B}_{21} \bm{B}_{11}^{-1} &= - \left( \bm{B}_{11}^{-1} \bm{B}_{12} \bm{F}_2^{-1} \right)^T \\
	&= -\sigma^{-2} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \bm{\phi}_i^T \P \Sxy \\
	\intertext{Substituting these quantities into the above expression for $\Sxy^{(\mathrm{new})}$, we have}
	\Sxy^{(\mathrm{new})} &= \left[ \begin{array}{cc} \Sxy + \sigma^{-4} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy & - \sigma^{-2} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \Sxy \P^T \bm{\phi}_i \\ -\sigma^{-2} \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \bm{\phi}_i^T \P \Sxy & \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \end{array} \right] \\
	&= \left[ \begin{array}{cc} \Sxy + \sigma^{-4} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy & - \sigma^{-2} \omega_i \Sxy \P^T \bm{\phi}_i \\ -\sigma^{-2} \omega_i \bm{\phi}_i^T \P \Sxy & \omega_i \end{array} \right]
\end{align}
where $\omega_i \triangleq \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1}$.

The expression for $\muxy^{(\mathrm{new})}$ can be expanded as
\begin{align}
	\muxy^{(\mathrm{new})} &= \sigma^{-2} \Sxy^{(\mathrm{new})} \left[ \begin{array}{cc} \P & \bm{\phi}_i \end{array} \right]^T \y \\
	&= \sigma^{-2} \left[ \begin{array}{cc} \Sxy + \sigma^{-4} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy & - \sigma^{-2} \omega_i \Sxy \P^T \bm{\phi}_i \\ - \sigma^{-2} \omega_i \bm{\phi}_i^T \P \Sxy & \omega_i \end{array} \right] \left[ \begin{array}{c} \P^T \\ \bm{\phi}_i^T \end{array} \right] \y \\
	&= \sigma^{-2} \left[ \begin{array}{c} \Sxy \P^T + \sigma^{-4} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy \P^T - \sigma^{-2} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \\ - \sigma^{-2} \omega_i \bm{\phi}_i^T \P \Sxy \P^T + \omega_i \bm{\phi}_i^T \end{array} \right] \y \\
	&= \left[ \begin{array}{c} \sigma^{-2} \Sxy \P^T \y + \sigma^{-6} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \P \Sxy \P^T \y - \sigma^{-4} \omega_i \Sxy \P^T \bm{\phi}_i \bm{\phi}_i^T \y \\ - \sigma^{-4} \omega_i \bm{\phi}_i^T \P \Sxy \P^T \y + \sigma^{-2} \omega_i \bm{\phi}_i^T \y \end{array} \right] \\
	&\triangleq \left[ \begin{array}{c} \left( \muxy^{(\mathrm{new})} \right)_1 \\ \left( \muxy^{(\mathrm{new})} \right)_2 \end{array} \right]
\end{align}
Evaluating these quantities, we have
\begin{align}
	\left( \muxy^{(\mathrm{new})} \right)_2 &= \omega_i \bm{\phi}_i^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \Sxy \P^T \right] \y \\
	&= \omega_i \bm{\phi}_i^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \y \\
	&= \omega_i \bm{\phi}_i^T \left( \sigma^2 \bm{I} + \P \G \P^T \right)^{-1} \y \\
	&= \omega_i \bm{\phi}_i^T \bm{C}^{-1} \y \\
	&= \omega_i Q_i \\
	\left( \muxy^{(\mathrm{new})} \right)_1 &= \muxy + \sigma^{-2} \Sxy \P^T \bm{\phi}_i \left( \muxy^{(\mathrm{new})} \right)_2 \\
	&= \muxy + \sigma^{-2} \omega_i Q_i \Sxy \P^T \bm{\phi}_i
\end{align}
so
\begin{align}
	\muxy^{(\mathrm{new})} &= \left[ \begin{array}{c} \left( \muxy^{(\mathrm{new})} \right)_1 \\ \left( \muxy^{(\mathrm{new})} \right)_2 \end{array} \right] = \left[ \begin{array}{c} \muxy + \sigma^{-2} \omega_i Q_i \Sxy \P^T \bm{\phi}_i \\ \omega_i Q_i \end{array} \right].
\end{align}

The expressions for $S_k^{(\mathrm{new})}$ and $Q_k^{(\mathrm{new})}$ can be obtained as
\begin{align}
	S_k^{(\mathrm{new})} &= \bm{\phi}_k^T \left( \bm{C}^{\mathrm{new}} \right)^{-1} \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \P \G \P^T + \bm{\phi}_i \widetilde{\gamma_i} \bm{\phi}_i^T \right)^{-1} \bm{\phi}_k \\
	&= \bm{\phi}_k^T \left[ \bm{C}^{-1} - \bm{C}^{-1} \bm{\phi}_i \left( \widetilde{\gamma_i} + \bm{\phi}_i^T \bm{C}^{-1} \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \bm{C}^{-1} \right] \bm{\phi}_k \\
	&= \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_k - \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \left( \widetilde{\gamma_i}^{-1} + \bm{\phi}_i^T \bm{C}^{-1} \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \bm{C}^{-1} \bm{\phi}_k \\
	&= S_k - \frac{\left( \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \right)^2}{\widetilde{\gamma_i}^{-1} + S_i} \\
	&= S_k - \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \left[ \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \P \G \P^T \right)^{-1} \bm{\phi}_i \right]^2 \\
	&= S_k - \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \left[ \bm{\phi}_k^T \left( \sigma^{-2} \bm{I} - \sigma^{-2} \bm{I} \P \left( \G^{-1} + \P^T \sigma^{-2} \bm{I} \P \right)^{-1} \P^T \sigma^{-2} \bm{I} \right) \bm{\phi}_i \right]^2 \\
	&= S_k - \left( \widetilde{\gamma_i}^{-1} + S_i \right)^{-1} \left[ \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_i - \sigma^{-4} \bm{\phi}_k^T \P \Sxy \P^T \bm{\phi}_i \right]^2 \\
	Q_k^{(\mathrm{new})} &= \bm{\phi}_k^T \left( \bm{C}^{(\mathrm{new})} \right)^{-1} \y \\
	&= \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \P \G \P^T + \bm{\phi}_i \widetilde{\gamma_i} \bm{\phi}_i^T \right)^{-1} \y \\
	&= \bm{\phi}_k^T \left[ \bm{C}^{-1} - \bm{C}^{-1} \bm{\phi}_i \left( \widetilde{\gamma_i}^{-1} - \bm{\phi}_i^T \bm{C}^{-1} \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \bm{C}^{-1} \right] \y \\
	&= \bm{\phi}_k^T \bm{C}^{-1} \y - \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \left( \widetilde{\gamma_i}^{-1} - \bm{\phi}_i - \bm{C}^{-1} \bm{\phi}_i \right)^{-1} \bm{\phi}_i^T \bm{C}^{-1} \y \\
	&= Q_k - \left( \widetilde{\gamma_i}^{-1} - S_i \right)^{-1} \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \bm{\phi}_i^T \bm{C}^{-1} \y \\
	&= Q_k - \left( \widetilde{\gamma_i}^{-1} - S_i \right)^{-1} \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \bm{\phi}_i^T \bm{C}^{-1} \y \\
	&= Q_k - \frac{Q_i}{\widetilde{\gamma_i}^{-1} - S_i} \bm{\phi}_k^T \bm{C}^{-1} \bm{\phi}_i \\
	&= Q_k - \frac{Q_i}{\widetilde{\gamma_i}^{-1} - S_i} \bm{\phi}_k^T \left( \sigma^2 \bm{I} + \P \G \P^T \right)^{-1} \bm{\phi}_i \\
	&= Q_k - \frac{Q_i}{\widetilde{\gamma_i}^{-1} - S_i} \bm{\phi}_k^T \left[ \sigma^{-2} \bm{I} - \sigma^{-4} \P \left( \G^{-1} + \sigma^{-2} \P^T \P \right)^{-1} \P^T \right] \bm{\phi}_i \\
	&= Q_k - \frac{Q_i}{\widetilde{\gamma_i}^{-1} - S_i} \left[ \sigma^{-2} \bm{\phi}_k^T \bm{\phi}_i - \sigma^4 \bm{\phi}_k^T \P \Sxy \P^T \bm{\phi}_i \right]
\end{align}

\subsubsection{Efficient updates for deleting an element}

\begin{align}
	\Sxy^{(\mathrm{new})} &= \Sxy - \left[ \frac{1}{0^{-1}-\gamma_i^{-1}} + \left(\Sxy\right)_{ii} \right]^{-1} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	&= \Sxy - \left[ \frac{1}{\infty-\gamma_i^{-1}} + \left(\Sxy\right)_{ii} \right]^{-1} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	&= \Sxy - \left[ \frac{1}{\infty} + \left(\Sxy\right)_{ii} \right]^{-1} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	&= \Sxy - \frac{1}{\left(\Sxy\right)_{ii}} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	\muxy^{(\mathrm{new})} &= \muxy - \left[ \frac{1}{0^{-1} - \gamma_i^{-1}} + \left(\Sxy\right)_{ii} \right]^{-1} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	&= \muxy - \frac{1}{\left(\Sxy\right)_{ii}} \left(\Sxy\right)_i \left(\Sxy\right)_i^T \\
	S_k^{(\mathrm{new})} &= S_k + \left[ \frac{1}{0^{-1} - \gamma_i^{-1}} + \left(\Sxy\right)_ii \right]^{-1} \left( \sigma^{-2} \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	&= S_k + \frac{1}{\left(\Sxy\right)_{ii}} \left( \sigma^{-2} \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \right)^2 \\
	Q_k^{(\mathrm{new})} &= Q_k + \left[ \frac{1}{0^{-1} - \gamma_i^{-1}} + \left(\Sxy\right)_{ii} \right] \left(\muxy\right)_i \left( \sigma^{-2} \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \right) \\
	&= Q_k + \frac{1}{\left(\Sxy\right)_{ii}} \left(\muxy\right)_i \left(\sigma^{-2} \left(\Sxy\right)_i^T \P^T \bm{\phi}_k \right)
\end{align}

\subsubsection{Full expressions for $\Delta_i$}

\begin{align}
	\Delta_j^{(\mathrm{add})} &= \ell(\widetilde{\gamma_j}) \\
	&= - \log \widetilde{\gamma_j}^{-1} + \log \left( \widetilde{\gamma_j}^{-1} + s_j \right) - \frac{q_j^2}{\widetilde{\gamma_j}^{-1} + s_j} - 2 a_j \log \widetilde{\gamma_j}^{-1} + 2 b_j \widetilde{\gamma_j}^{-1} \\
	&= \log \left[ \frac{\widetilde{\gamma_j}^{-1} + s_j}{\widetilde{\gamma_j}^{-1}} \right] - \frac{q_j^2}{\widetilde{\gamma_j}^{-1} + s_j} + 2 a_j \log \widetilde{\gamma_j} + 2 b_j \widetilde{\gamma_j}^{-1} \\
	&= \log \left[ 1 + s_j \widetilde{\gamma_j} \right] - \frac{q_j^2}{\widetilde{\gamma_j}^{-1} + s_j} + 2 a_j \log \widetilde{\gamma_j} + 2 b_j \widetilde{\gamma_j}^{-1} \\
	\Delta_j^{(\mathrm{delete})} &= -\ell(\gamma_j) \\
	&= \log \gamma_j^{-1} - \log \left( \gamma_j^{-1} + s_j \right) + \frac{q_j^2}{\gamma_j^{-1} + s_j} - 2 a_j \log \gamma_j - 2 b_j \gamma_j^{-1} \\
	&= \log \left[ \frac{\gamma_j^{-1}}{\gamma_j^{-1} + s_j} \right] + \frac{q_j^2}{\gamma_j^{-1} + s_j} - 2 a_j \log \gamma_j - 2 b_j \gamma_j^{-1} \\
	&= \log \left[ \frac{1}{1 + \gamma_j s_j} \right] + \frac{q_j^2}{\gamma_j^{-1} + s_j} - 2 a_j \log \gamma_j - 2 b_j \gamma_j^{-1} \\
	&= - \log \left[ 1 + s_j \gamma_j \right] + \frac{q_j^2}{\gamma_j^{_1} + s_j} - 2 a_j \log \gamma_j - 2 b_j \gamma_j^{-1} \\
	\Delta_j^{(\mathrm{re-est})} &= \ell\left(\widetilde{\gamma_j}\right) - \ell\left(\gamma_j\right) \\
	&= - \log \widetilde{\gamma_j}^{-1} + \log \gamma_j^{-1} + \log \left( \widetilde{\gamma_j}^{-1} + s_j \right) - \log \left( \gamma_j^{-1} + s_j \right) - \frac{q_j^2}{\widetilde{\gamma_j}^{-1} + s_j} + \frac{q_j^2}{\gamma_j^{-1} + s_j} - 2 a_j \log \widetilde{\gamma_j}^{-1} + 2 a_j \log \gamma_j^{-1} + 2 b_j \widetilde{\gamma_j}^{-1} - 2 b_j \gamma_j^{-1} \\
	&= \log \left[ \frac{\gamma_j^{-1}}{\widetilde{\gamma_j}^{-1}} \frac{\widetilde{\gamma_j}^{-1} + s_j}{\gamma_j + s_j} \right] + q_j^2 \left( \frac{1}{\gamma_j^{-1} + s_j} - \frac{1}{\widetilde{\gamma_j}^{-1} + s_j} \right) + 2 a_j \log \left( \frac{\gamma_j^{-1}}{\widetilde{\gamma_j}^{-1}} \right) + 2 b_j \left( \widetilde{\gamma_j}^{-1} - \gamma_j^{-1} \right) \\
	&= \log \left[ \frac{\widetilde{\gamma_j}}{\gamma_j} \frac{\widetilde{\gamma_j}^{-1} + s_j}{\gamma_j^{-1} + s_j} \right] + q_j^2 \left( \frac{1}{\gamma_j^{-1} + s_j} - \frac{1}{\widetilde{\gamma_j}^{-1} + s_j} \right) + 2 a_j \log \left( \frac{\widetilde{\gamma_j}}{\gamma_j} \right) + 2 b_j \left( \widetilde{\gamma_j}^{-1} - \gamma_j^{-1} \right)
\end{align}
